Hidden Gems: 4D Radar Scene Flow Learning Using Cross-Modal Supervision

This work proposes a novel approach to 4D radar-based scene flow estimation via cross-modal learning. Our approach is motivated by the co-located sensing redundancy in modern autonomous vehicles. Such redundancy implicitly provides various forms of supervision cues to the radar scene flow estimation. Specifically, we introduce a multi-task model architecture for the identified cross-modal learning problem and propose loss functions to opportunistically engage scene flow estimation using multiple cross-modal constraints for effective model training. Extensive experiments show the state-of-the-art performance of our method and demonstrate the effectiveness of cross-modal supervised learning to infer more accurate 4D radar scene flow. We also show its usefulness to two subtasks - motion segmentation and ego-motion estimation. Our source code will be available on https://github.com/Toytiny/CMFlow.

==> section/method_old.tex <==
The overall pipeline of our approach is depicted in~\cref{fig:pipeline}. Given multi-modal training data, we first generate task-specific supervision signals from three modalities individually. Then, we investigate how to fuse some of them before we feed them to our trainer. More details about our cross-modal supervision extraction and fusion will be illustrated in~\cref{cross-modal}. 

Our cross-modal supervision signals include a) the ego-motion transform, rigid flow components and a pseudo motion segmentation mask label generated with the odometry information, b) the pseudo foreground segmentation mask label and foreground scene flow labels obtained with the LiDAR point clouds, c) the point-wise pseudo optical flow labels estimated from the monocular images from RGB camera. 

Our model architecture is designed based on~\cite{ding2022raflow} \chris{@FQ, You should not make such a direct deduction here about our relationship with Raflow. This work should be self-contained. Moreover, it violates the double-blind policy.} but we induce non-trivial changes to render it compatible with our cross-modal supervision framework (c.f.~\cref{model}). The outputs of our model are composed of the refined scene flow prediction, the estimated radar ego-motion transform and the point-wise motion classification scores. To constrain these predictions during training, we formulate multiple loss functions in~\cref{loss} using supervision signals extracted from cross-modalities. In the last, we propose a GRU-based global feature updating module that can be embedded in the backbone for leveraging temporal information from previous frames (c.f.~\cref{temporal}). 

%Maybe can be used in the introduction section
%\noindent \textbf{Supervision Extraction.} With the odometry information, we compute the ego-motion transform between two frames and derive the rigid flow component of each point in the source frame. The rigid flow components are further used together with the RRV measurements to generate pseudo motion segmentation labels.  With dense point clouds captured from LiDAR, we apply off-the-shelf 3D multi-object tracking algorithms to obtain pseudo bounding boxes and their associated ID labels. By identifying inbox points and apply associated box transformation, pseudo foreground (FG) segmentation labels and the pseudo scene flow labels of FG points can be calculated. Given the monocular images from RGB camera, the pretrained optical flow model is deployed to the pseudo optical flow maps for the whole source image. 

\begin{figure*}[tbp!]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/simplified_pipeline.pdf}
    \caption{Overall pipeline of our cross-modal supervised learning of 4D radar scene flow estimation. \chris{@FQ, please redraw this one. }}
    \label{fig:pipeline}
\end{figure*}
\subsection{Cross-Modal Supervision}\label{cross-modal}
For autonomous vehicles, different sensors afford various perception functionalities and constitute a crucial part of safe navigation. To emulate the real scenarios of autonomous driving and support the development of reliable perception systems, many public datasets~\cite{geiger2013vision,caesar2020nuscenes, sun2020scalability,palffy2022multi} collect multi-modal data with complementary sensor types. Among them, odometer, LiDAR and RGB camera are the most common sensors used in multi-modal autonomous driving datasets. We, therefore, exploit these three sensors to extract cross-modal supervision for learning scene flow estimation on 4D radar point clouds. 

\vspace{0.5em}
\noindent \textbf{Supervision from Odometer.} As a key sensor for mobile autonomy, the odometer is responsible for tracking the position and rotation of ego-vehicles, which is commonly the combination of RTK-GPS and IMU. To utilize the odometry information, we first compute the radar ego-motion transform $\mathbf{O}\in\mathbb{R}^{4\times 4}$ between two point clouds using the ego-vehicle pose at two keyframes and radar extrinsic parameters. A rigid transformation matrix $\mathbf{T}=\mathbf{O}^{-1}$ can be then derived to summarize the rigid flow component $\mathbf{F}^{r}=\{\mathbf{f}_{i}^{r}\}_{i=1}^{N}$ induced by radar ego-motion. For each point in $\mathbf{P}^s$, the rigid part of its scene flow can be obtained by $[\mathbf{f}_{i}^{r}~1]^{\top} = (\mathbf{T}-\mathbf{I}_4)[\mathbf{c}_i^s~1]^{\top}$. $\mathbf{T}$ can be seen as a prediction target to supervise our training through the ego-motion loss function (c.f. \cref{loss:ego}), while $\mathbf{F}^{r}$ can be used for signal fusion and generating the pseudo segmentation label below.

The relationship between the RRV measurement $v_i$ and scene flow vector $\mathbf{f}_i$ is established in~\cite{ding2022raflow} as:  
\begin{equation}\label{rrv}
    v_i{\Delta t} \approx {\mathbf{u}_i^\top \mathbf{f}_i}
\end{equation}
where $\mathbf{u}_i$ is the unit vector with its direction pointing from the sensor to the point $\mathbf{c}^s_i$. $\Delta t$ is time duration between two frames and is short enough (\eg 0.1s) so that the point velocity can be approximately regarded as constant.  Substituting rigid flow component $\mathbf{f}^r_i$ to~\cref{rrv}, the RRV component $v_i^{r}$ ascribed to the radar ego-motion can be first derived. Then we compensate the radar ego-motion and get the object absolute radial velocity $\Delta v_i = \mathrm{abs}(v_i-v_i^r)$. 

With per-point $\Delta v_i$, it is intuitive to generate a motion segmentation mask by labeling points with larger values than a fixed threshold as moving points. However, this vanilla strategy suffers from the temporal asynchronization between the well-curated keyframes  and original radar point clouds.  Even though the coordinates of radar points are transformed to the timestamp of keyframes using high-frequency odometry information, their RRV measurements still corresponds to the original timestamps.  As a result, there is often a non-trivial global bias in $\Delta v_i$, which disturbs the identification of real moving points given a fixed threshold. For example, almost all points could be classified as moving when a large bias exists. 

To mitigate this issue, we propose to normalize all $\Delta v_i$ by subtracting the mean value $\mu$ of them and then classify points by thresholding. The pseudo motion segmentation label $\mathbf{S}^{v}=\{s_i^{v}\in\{0,1\}\}_{i=1}^{N}$ can then be created with a fixed threshold $\eta_v$,
%\begin{equation}
%    s_i^v = 
%    \left\{
%    \begin{aligned}
%    0, &\quad \mathrm{if}~\Delta v_i - \mu < \eta_v\\
%    1, &\quad \mathrm{else}
%    \end{aligned}
%    \right.
%\end{equation}
%where 0 represents stationary points. We determine the value of $\eta_v$ via grid searching on the validation set. More details can be seen in the supplement materials. 
%By compensating the global bias, our strategy can effectively avoid the circumstances that many static points are mistakenly labelled as moving and improve the quality of our pseudo motion segmentation labels. 
%As a important supervision signal, $\mathbf{S}^v$ can be used to supervise the estimation of motion segmentation after the signal fusion stage.
%\vspace{0.5em}

%\noindent\textbf{Supervision from LiDAR.} As another active sensor, LiDAR can detect targets and measure their 3D positions by emitting pulsed lasers~\cite{li2020lidar}. Compared with 4D radar, it can restore the geometric structure well with denser point data under satisfactory weather conditions. Some recent works~\cite{weng20203d,weng2020gnn3dmot,yin2021center} perform 3D multi-object tracking (MOT) on LiDAR point clouds in a \emph {tracking-by-detection} paradigm and show prominent results. Inspired by the progress, we propose to exploit supervision signals from LiDAR through running 3D MOT algorithms on LiDAR point clouds.

%As the foremost step, a sequence of LiDAR point clouds are fed into off-the-shelf 3D MOT pretrained models. The outputs are oriented 3D bounding boxes and their track IDs at each frame. These object-level results are then transformed from the LiDAR to the radar coordinate frame and assigned to each radar point cloud. Since the whole scene is divided into the foreground and background by predicted bounding boxes, a pseudo foreground segmentation label $\mathbf{S}^{fg}=\{s_i^{fg}\in\{1,0\}\}_{i=1}^{N}$ can be readily obtained for the source point cloud $\mathbf{P}^s$, where 1 is the mark for foreground points.
%To aggregate point-wise scene flow supervision for $\mathbf{P}^s$, we first individually compute the inter-frame transformation for each bounding box in the first frame by retrieving the same ID in the second frame.  Then we compute the translation vector for each inbox point in $\mathbf{P}^s$ based on the assumption that all points belonging to the same object share a \emph{universal} rigid transformation. With this labeling scheme, all inbox (\emph{aka.} foreground) points in  $\mathbf{P}^s$ are assigned their own pseudo scene flow labels, denoted as $\mathbf{F}^{fg}=\{\mathbf{f}_i^{fg}\}_{i=1}^{N}$, where we leave the label empty for all identified background points. As the two labels obtained from LiDAR are both for the foreground, we distil the moving part from them during signal fusion before we use them.

%\vspace{0.5em}
%\noindent \textbf{Supervision from RGB Camera.}
%Different from LiDAR or radar point
%clouds, RGB images contain explicit object appearance and texture information, which provide rich semantics cues for inferring pixel-level 2D motions between frames, \ie optical flow estimation. As a 2D perspective projection of 3D scene flow, optical flow describes the motion of points on the image plane. Thus it can also be used to weakly supervise the scene flow estimation of points, whose perspective projection is within the camera field-of-view (FoV). Thanks to the advance on data-driven optical flow estimation~\cite{teed2020raft,sun2018pwc}, we can use pretrained model to infer pseudo optical flow label efficiently. For one pair of $\mathbf{P}^s$ and $\mathbf{P}^t$, we input their synchronized monocular images $\mathbf{I}^s$ and $\mathbf{I}^t$ into the network and obtain a optical flow map. After projecting all radar points in $\mathbf{P}^s$ to the image plane, the pseudo optical flow label associated to each radar point can then be drawn, denoted by $\bar{\mathbf{W}}=\{\bar{\mathbf{w}}_i\}_{i=1}^{N}$. %Note that we only extract the optical flow vector for radar points within the camera FoV. 
%As the only supervision mined from RGB camera, the pseudo optical flow label is used to constrain the scene flow prediction in the optical flow loss (c.f.~\cref{loss:opt})

%\vspace{0.5em}
%\noindent \textbf{Supervision Signal Fusion.} After extracting various supervision signals from individual modalities, we conduct a fusion step before forwarding them to guide the training phase. The motivation behind this process is that we have two pseudo segmentation labels in hand, the pseudo foreground segmentation label $\mathbf{S}^{fg}$ from LiDAR and motion segmentation label $\mathbf{S}^{v}$ from odometer, which can potentially be fused. However, the domain gap between them impedes the direct fusion. To overcome it, we propose to distill the moving part from $\mathbf{S}^{fg}$ by discarding foreground points that either keep still or moves very slowly. 

%In concrete, we first remove the rigid flow component $\mathbf{F}^r$ from the pseudo foreground flow label $\mathbf{F}^{fg}$ to derive the non-rigid flow component $\mathbf{f}_i^{fg}-\mathbf{f}_i^{r}$ of all foreground points indicated in $\mathbf{S}^{fg}$. Then we generate a new pseudo motion segmentation label $\mathbf{S}^{l} = \{{s}_i^{l}\in\{0,1\}\}_{i=1}^{N}$ by classifying points with apparent non-rigid flow as dynamics. A more reliable pseudo motion segmentation $\bar{\mathbf{S}}=\{\bar{s}_i\}_{i=1}^{N}$ can be consequently obtained by fusing $\mathbf{S}^{l}$ and $\mathbf{S}^{v}$ appropriately.
%\begin{equation}\label{fuse}
%    \bar{s}_i = 
%    \left\{
%    \begin{aligned}
%    1, &\quad \mathrm{if}~s_i^l = 1 \\
%    s^v_i, &\quad \mathrm{else}
%    \end{aligned}
%    \right.
%\end{equation}
%For points classified as dynamics in $\mathbf{S}^{l}$, we have a high confidence in their status because they are not only tracked by MOT algorithms but have non-rigid flow components in their pseudo scene flow labels. Thus, we label these points as moving in $\bar{\mathbf{S}}$. However, we are not certain about the status of points identified as stationary in $\mathbf{S}^{l}$, because some of them may come from false negative of MOT results. We use the label values from $\mathbf{S}^{v}$ for these points. Apart from $\mathbf{S}^{l}$, we also draw the moving part from the pseudo foreground flow label $\mathbf{F}^{fg}$ and denote it as $\mathbf{F}^{l} = \{\mathbf{f}_i^{l}\}_{i=1}^{N}$, where only the labels for moving points are valid. 

%\subsection{Model Architecture}\label{model}
%Similar to the network in~\cite{ding2022raflow, baur2021slim,tishchenko2020self}, we apply a two-stage fashion in our model architecture. In the first stage, we generate a flow embedding through the backbone and predict a basic scene flow and a motion classification logit map using two separate MLP-based heads. The second stage first estimates the radar ego-motion transform between two frames and then refines the scene flow of static points with it. We introduce more details of different components as follows. 
%\vspace{0.5em}

%\noindent\textbf{Scene Flow Backbone.} Following~\cite{ding2022raflow}, we encode point-wise features of two input point clouds, $\mathbf{P}^s$ and $\mathbf{P}^t$, by multi-scale~\emph{set conv} layers~\cite{liu2019flownet3d} and propagate features from $\mathbf{P}^t$ to $\mathbf{P}^s$ using the~\emph{cost volume} layer~\cite{wu2020pointpwc}. We then concatenate multi-stage features of $\mathbf{P}^s$ and forward them into another multi-scale $\emph{set conv}$ layers to generate the flow embedding $\mathbf{E}\in\mathbb{R}^{N\times 512}$. See the supplementary material for more layer details of the backbone.
%\vspace{0.5em}

%\noindent\textbf{Scene Flow \& Motion Segmentation Head.} Given the flow embedding $\mathbf{E}$ that represents the inter-frame motion and intra-frame local-global information for each point in $\mathbf{P}^s$, we apply two task-specific heads for decoding. The first head is to produce a basic scene flow $\hat{\mathbf{F}}^{b}=\{\hat{\mathbf{f}}_i^b\in\mathbb{R}^3\}_{i=1}^N$, while another is for generating a logit map $\hat{\mathbf{S}}=\{\hat{s}_i\in[0,1]\}_{i=1}^N$ that denotes the moving probabilities of points (\emph{w.r.t.} the world frame). Both heads are implemented by the MLP that has three hidden layers whose width is $[256, 128, 64]$.
%\vspace{0.5em}

\noindent\textbf{Ego-Motion Head.} With the natural correspondences $\{\mathbf{c}^s_i,\mathbf{c}^s_i+\hat{\mathbf{f}}_i\}_{i=1}^N$ formed by the basic scene flow $\hat{\mathbf{F}}^b$, we can restore a rigid transformation $\hat{\mathbf{T}}$ that represents radar ego-motion using the differentiable weighted Kabsch algorithm~\cite{kabsch1976solution}. To mitigate the influence of the flow vectors from high-potential moving points, we compute $1-\hat{\mathbf{S}}$ as our weights and normalize the sum of all weights to 1. Besides, a binary motion segmentation mask can be created from $\hat{\mathbf{S}}$ given a fixed threshold $\eta_b$. We use this binary mask as our motion segmentation output and to identify stationary points for flow refinement as follows.  In particular, for the ego-motion head, we use the pseudo label $\bar{\mathbf{S}}$ instead of $\hat{\mathbf{S}}$ in the training stage for a stable learning of scene flow. 
\vspace{0.5em}

\noindent\textbf{Refinement Layer.} As the flow vectors of static points only have the rigid component caused by the radar ego-motion, we can regularize them with the estimated rigid transformation $\hat{\mathbf{T}}$. The refinement operation is simply replacing the basic flow vector $\hat{\mathbf{f}_i^b}$ of identified stationary points with $\hat{\mathbf{f}_i}$ derived by $[\hat{\mathbf{f}_i}~1]^{\top}=(\hat{\mathbf{T}}-\mathbf{I}_4)[\mathbf{c}_i^s~1]^{\top}$. We denote the final scene flow as $\hat{\mathbf{F}}=\{\hat{\mathbf{f}}_i\in\mathbb{R}^3\}_{i=1}^N$

\subsection{Loss}\label{loss}
To guide the end-to-end training of our model, we formulate different loss functions using cross-modal supervision signals, which are illustrated in the following details. 
\vspace{0.5em}

\noindent \textbf{Motion segmentation loss.}
We apply the pseudo binary motion segmentation label $\bar{\mathbf{S}}$ to constrain the predicted logit map $\hat{\mathbf{S}}$ used for motion segmentation:
\begin{equation}\label{loss:seg}
    \mathcal{L}_{seg} = \frac{1}{2}( \frac{\sum_{i}(1-\bar{s}_i)\mathrm{log}(1-\hat{s}_i)}{\sum_{i}(1-\bar{s}_i)} +\frac{\sum_{i}\bar{s}_i\mathrm{log}(\hat{s}_i)}{{\sum_{i}\bar{s}_i}})
\end{equation}
Here, we use the average loss between losses from the static and moving points to address the class imbalance issue. 
\vspace{0.5em}

\noindent \textbf{Ego-motion loss.}
With the rigid transform $\mathbf{T}$ given by the odometer, we supervise the ego-motion output $\hat{\mathbf{T}}$ through:
\begin{equation}\label{loss:ego}
    \mathcal{L}_{ego} = \frac{1}{N} \sum_{i=1}^{N}||(\mathbf{\hat{T}}-\mathbf{{T}})
    [\mathbf{c}_i^s~1]^{\top}
    ||_2
\end{equation}
By supervising $\hat{\mathbf{T}}$, we can implicitly constrain the basic scene flow $\hat{\mathbf{f}}^b_i$ from identified static points according to $\hat{\mathbf{S}}$. The final flow $\hat{\mathbf{f}_i}$ of those points are also supervised as their flow refinement is based on $\hat{\mathbf{T}}$.
\vspace{0.5em}

\noindent \textbf{Moving Flow loss.} Different from the static flow vectors that are implicitly supervised by the ego-motion loss, the flow vectors of those moving points identified by $\mathbf{S}^l$ are directly constrained by the pseudo label $\mathbf{F}^l$ through:
\begin{equation}\label{loss:mov}
    \mathcal{L}_{mov} = \frac{1}{\sum_{i}{s_i^l}}\sum_{i=1}^{N}||{s}^{l}_i(\mathbf{\hat{f}}_i-\mathbf{f}^{l}_i)||_2
\end{equation}
%Here, for moving points that are identified by $\mathbf{S}^v$ but not by $\mathbf{S}^l$ (c.f.~\cref{fuse}), their flow vectors can not be supervised. 
\vspace{0.5em}

\noindent \textbf{Optical Flow Loss.}
Given pseudo optical flow label $\bar{\mathbf{W}}$ estimated from corresponding images, it is intuitive to construct the supervision for scene flow by projecting it on the image plane. However, minimizing the flow divergence in pixel scale has less impact for far radar points due to the depth-unawareness during perspective projection. 
%As seen in Figure~\ref{fig:optical}, a larger distance between the warped point $\mathbf{q}^1_{j}$ and the expected ray $l_j$ results in a smaller pixel-scale loss after perspective projection for a farther point.
Instead, we directly take the point-to-ray distance as the training objective, which is more insensitive to points at different ranges. The loss function can be formulated as:
\begin{equation}\label{loss:opt}
    \mathcal{L}_{opt} = \frac{1}{\sum_{i}\bar{s}_i}\sum_{i=1}^{N}\bar{s}_i\mathcal{D}(\mathbf{c}^s_i+\mathbf{\hat{f}}_i, \mathbf{m}_i+\mathbf{w}_i;\theta)
\end{equation}
where $\mathcal{D}$ denotes the operation that computes the distance between the warped point $\mathbf{c}^s_i+\mathbf{\hat{f}}_i$ and the ray $l_i$ traced from the warped pixel $\mathbf{m}_i+\mathbf{w}_i$. $\theta$ denotes  sensor calibration parameters. We only consider the scene flow of moving points here as the static flow vectors are supervised well in~\cref{loss:ego}.
\vspace{0.5em}

\noindent \textbf{Total loss.} Apart from the above loss functions powered by cross-modal supervision, we also leverage the self-supervised one proposed in~\cite{ding2022raflow} as complement to our loss. Combing our loss components, the total loss can be written as:
\begin{equation}\label{loss:tot}
    \mathcal{L}_{tot} = \mathcal{L}_{self} + \mathcal{L}_{seg} + \mathcal{L}_{ego} + \mathcal{L}_{mov} + \alpha\mathcal{L}_{opt}
\end{equation}
where $\alpha:=0.1$ is used for all experiments as the weight. \chris{@FQ, so the weight of each cross-modal supervision signal is always 1 in our case?}

\subsection{Temporal Feature Update Module}\label{temporal}
\chris{bad place to put this module here abruptly. It should go into the model archi. My question is that - is this temporal module novel enough to spend this long paragraph? Do any other works re. scene flow estimation have similar recurrent neural network usage for scene flow estimation?} 
In the traditional paradigm, a sequence of point clouds is processed by feeding each pair of two consecutive frames into the model and estimate the scene flow independently. This paradigm breaks the connection between current and previous frames, and automatically ignores the temporal information. Given sequences of temporal data, it is intuitive to exploit temporal signals to benefit scene flow estimation. To this end, we add a GRU-based module into our framework for updating features temporally along the sequence.

Unlike image grids that have regular input data formats, and fixed data volume, point clouds are unordered sets of points and have various numbers of points. As a result, local point-level features have uncertain dimensions, and points with the same index are not spatially corresponding across frames. Given this, we propose to update the scene global feature instead of local point-level features. 

Before forming the final embedding in our backbone, we apply a max-pooling onto point-level features and obtain a global feature vector $\mathbf{G}^{t}\in\mathbb{R}^{256}$. Taking the $\mathbf{G}^{t}$ as current iteration information, given the previous hidden state $\mathbf{H}^{t-1}\in\mathbb{R}^{256}$, we use a GRU cell to produce an updated hidden state $\mathbf{H}^{t}$. The final embedding from the backbone can be generated by expanding $\mathbf{H}^{t}$ for $N$ times along the point axis and concatenating it with the point-level features. 

During training, to avoid overfitting on long sequences,  we first split long training sequences into short clips with a fixed length $T$ and train with mini-batches of clips. The hidden state is initialized as zero vector for the first frame. When evaluating on long sequence, we emulate the training process by re-initializing the hidden state after $T$ frames.
